Personhood Credentials: Human-Centered Design Recommendation Balancing Security, Usability, and Trust

Building on related concepts, like, decentralized identifiers (DIDs), proof of personhood, anonymous credentials, personhood credentials (PHCs) emerged as an alternative approach, enabling individuals to verify to digital service providers that they are a person without disclosing additional information. However, new technologies might introduce some friction due to users misunderstandings and mismatched expectations. Despite their growing importance, limited research has been done on users perceptions and preferences regarding PHCs. To address this gap, we conducted competitive analysis, and semi-structured online user interviews with 23 participants from US and EU to provide concrete design recommendations for PHCs that incorporate user needs, adoption rules, and preferences. Our study -- (a)surfaces how people reason about unknown privacy and security guarantees of PHCs compared to current verification methods -- (b) presents the impact of several factors on how people would like to onboard and manage PHCs, including, trusted issuers (e.g. gov), ground truth data to issue PHC (e.g biometrics, physical id), and issuance system (e.g. centralized vs decentralized). In a think-aloud conceptual design session, participants recommended -- conceptualized design, such as periodic biometrics verification, time-bound credentials, visually interactive human-check, and supervision of government for issuance system. We propose actionable designs reflecting users preferences.

==> Sections/Pilot/Results_RQ1_pilot.tex <==
\section{RQ1: Users’ perception of PHC}

\subsection{Current Online Identity Verification Practices}

\textbf{Verification Across Multiple Domains} The most common online services where participants encountered identity verification processes are financial services, including online banking and investment platforms. Several participants mentioned they are required to upload government IDs (e.g., social security number, driver's license) when creating an account; as P1 said, \textit{"I use the bank I need to upload my social security number for, such as PNC Bank and Discover. I don't really remember. But I'm sure I have uploaded my social security number."} In addition to financial services, the typical applications where participants experienced verification or authentication processes include social media, government services, and healthcare platforms. 
%This indicates that the scenarios we prepared for succeeding sessions are representative of typical user occasions. 

\textbf{Confusion Between Verification and Authentication} Many participants did not distinguish between verification and authentication. In particular, when asked about experiences with biometric verification, they often shared daily experiences related to authentication, e.g., (P3): \textit{"It's I think most of the apps required me such fingerprints or related identification. For example, when I open my bank apps, I can just use my fingers to login to my account."} Participants indicated frequent use of fingerprints or face authentications on mobile phones. For instance, P1 mentioned stored biometric information on devices, \textit{"Because my android phone already have my fingerprint to log into my phone. And then this app just to reuse my fingerprint, which is already registered on my phone."}

\textbf{Verification in daily life} Some of the participants shared their offline experience that required identity verification, as P1 described \textit{"So I need to check in in a hotel. I also need to show my driver's license. I don't know if that count."} 

\subsection{Perceived Benefits of Personhood Credentials}
%\fixme{there needs to be titles of sub-themes under this benefit, it's hard to read. Sub-themes could be -- convenience of not carrying physical id, etc -- whatever unique /interesting subthemes came up in the interview}
\textbf{Reduced Exposure of Personal Information} Participants identified a range of benefits, the most frequently mentioned being the reduction of personal information exposure. P4 expressed their reassurance in unnecessary data sharing to online platforms, \textit{"I feel less concerned. Because there's a platform which is designed for keeping my information, and I don't have to keep my personal information to any online platform that I have I want to interact with. Probably it's gonna be easier."} In addition to this, several participants noted the benefits related to minimizing data leakage. P5 explained the potential for data linkability, where information from other datasets could be combined to identify, \textit{"We also have different problem privacy that they can have some of our information from another anonymized data set. They can point out our previous record. So this will probably make it safer."} Participants also extended the discussion on this point to online malicious attacks, \textit{"So for benefits, the overall perspective of this PHC will be like minimizing the exposure of personal information to open world. We have faced problems like fake accounts and misuse of social security numbers. It can be reduced because of PHC. "}

\textbf{Efficiency of Verification Process} Another key benefit highlighted by participants was the efficiency of verification process. P3 emphasized the convenience of only needing to verify their official documents once, stating, \textit{"So one of the benefits is convenienceness. Users only verified their official document only once, and then after that they can always use the token as PHCs, so that's very convenient." }


\subsection{Perceived Concerns of Personhood Credentials}
%\fixme{there needs to be titles of sub themes under this benefit, it's hard to read }
Participants expressed various concerns, primarily revolving around data security and trustworthiness of PHC issuers. 

\textbf{PHC Issuer Being Hacked or Leaked} One of the most frequently mentioned concerns was the potential risk of PHC issuers being hacked or experiencing data leaks. As P3 explained, \textit{"The issuer really matters. If the data leaks from the issuer and is stolen by someone, then you know every single information will be gone, which is a huge problem."} It highlights participants' fears that the concentration of sensitive data with PHC issuers could have severe consequences for malicious attacks.

\textbf{Data Handling by PHC Issuers} Another significant concern was how PHC issuers manage and handle the credential data they collected. Participants showed uncertainties regarding what happens to their personal information after verification and whether it is securely stored or potentially mishandled. For example, P4 shared that \textit{"I'm not sure if they tell us explicitly how they're gonna use, do they going to share our information with 3rd party or with government. If they ask for it, I'm not sure about that. These are my concerns."}

\textbf{Centralized Power of PHC Issuer} Several participants expressed concerns over the centralized power held by PHC issuers, which they feared could lead to misuse or overextension of control. P4 commented \textit{"But I think there's a concern on the other side that they're gonna be one kind of you're gonna give all your information to a small group or an institution. So they have the power that can be abused later."} illustrating the apprehension about the concentration of power in the hands of a single entity as a PHC issuer.

\textbf{Untrustworthy PHC Issuer} The issue of trustworthiness in PHC issuers was also discussed, with participants expressing doubts about the reliability of the entities managing their data. Some worried whether these issuers could be trusted to protect their personal information and maintain their privacy. P5 described \textit{"The problem is, and the whole thing comes like how much you can trust the PHC issuer. If it's associated with government, there can be a reduced risk associated with like...But if it's an overall 3rd party, people will be thinking like, is it true? Is it a scammer?"}

\subsection{Perception Before \& After Educational Video}
As discussed in the method section \ref{sec:study_protocol}, we revisited questions about participants' understanding of PHC to compare their responses before and after watching the educational video to assess whether the video impacted their original knowledge of PHC. 

\textbf{Pre-understanding: Guessed it as one of the verification methods} The majority of participants were unfamiliar with PHC. When prompted to interpret the term based solely on its wording, most inferred that it referred to a form of verification method. (e.g., P3 noted \textit{"I think this one probably be another type of person identification method."})

\textbf{Post-understanding: PHC improves privacy and security} When asked to explain their understanding of PHC, P3 noted, \textit{"Personhood credentials tries to define a more trusted 3rd party that we can verify personal information and get some like passport or credential. Then we use different online services that we don't know what the sources are."} This suggests that the role of the PHC issuer is recognized as a crucial component of PHC.

\textbf{Post-understanding: Found similarities with other technologies} P5 interpreted the term as a verification method based on personal characteristics, which differ from person to person, such as behavioral patterns, commenting \textit{"It's like, personality based or like activities humans particularly perform. It sounds similar to the pattern of people walking. Those are also things people use for verification."} After watching the video, he updated his perception of PHC \textit{"I thought it was similar to SSL technology. Like in SSL, they will give the certificate to 3rd party who encrypts and has those certificates. To maintain their integrity, they will pass on the kind of certificate to web browsers. So when a user goes through a particular website, they will be able to cross-verify using the public keys available."}, linking it to technologies such as SSL, which uses encryption and hashing for certificates.


==> Sections/Pilot/Results_RQ2_pilot.tex <==
\section{RQ2: Users’ preference of PHC}

\subsection{Preferred Credential Types}
Participants' preferred credential types can be categorized into three main verification methods: \ding{202} Government-issued IDs, such as social security numbers, passports, and driver's licenses; \ding{203} Biometrics, including face and fingerprints; and \ding{204} Digital identifiers, such as phone numbers and email addresses.

\textbf{Ease of Biometrics Over Government IDs} While concerns about the risk of data leaks were expressed regarding government-issued IDs, the convenience of biometric authentication was emphasized. For instance, P2 mentioned \textit{"I think this information may be lost, or maybe stolen by other people. So it's a risk. Think the passport and the ID card."} It underscores that participants worry about the potential vulnerability of physical IDs. At the same time, P2 showed their preference for biometrics, stating \textit{"I think fingerprint authentication is much easier than other methods because I don't have to remember passwords or complex PINs. I just use my fingerprints. It's much easier." } 

\textbf{Trade-off on Digital Identifiers} Participants also shared their preference with a trade-off on digital identifiers, noting both risks and advantages. P3 acknowledged the potential risks with \textit{"Email address is more likely leaked or stolen by other people. So I think it has many risks related to using an email address."} However, P3 preferred using an email address as a credential, supplementing by \textit{"But on the other hand, an email address will not leak my personal information too much. so I think, for the pros and cons, I like this."} 

\subsection{Preferred Stakeholder Types}
\textbf{Differing Trust Across Stakeholders}
Participants expressed different levels of trust depending on the type of stakeholder. Key insights include relatively higher trust in the government, contrasted with a pronounced distrust regarding social media privacy. P2 noted their confidence in the government: \textit{"I trust the government. The government already have this information. So it's okay. "} It showed preference in handling sensitive information. They further explained that they did not extend the same trust to private companies or organizations, particularly social media platforms. P2 expressed their concerns, stating \textit{"I think, for social media companies, they may not secure as secure as a financial system. I read some news that many big companies leaks their customers' information. So I think it's not okay to provide my passport or my that kind of information to the company."} This contrast highlights the complex considerations individuals have when evaluating trust in different entities for managing private data.

\textbf{Variability in Trust Among Individuals}
While there was a general consensus on preferred entities for data trust, individual perspectives varied regarding which organizations were considered trustworthy. For example, P4 expressed distrust toward the government, commenting \textit{"Government is not kind of trying to protect most of the citizens’ privacy and security, but at the same time it’s going to give more power to the government."} They also showed relative trust in social media companies, explaining \textit{"They probably invest in the privacy and security part. So I’m kind of less concerned."} These contrasting viewpoints highlight how personal beliefs and experiences shape individual trust preferences, underscoring the diversity of opinion in stakeholder trust.


\subsection{Context Matters for Users' Preference}
As outlined in the method section \ref{sec:study_protocol}, we explored participants’ perceptions and preferences regarding PHC across five distinct scenarios. 

\textbf{Unnecessary PHC Use in Specific Scenarios} Participants’ responses indicated the necessity of verification methods depending on the specific scenario.  In some contexts, they considered PHC unnecessary and suggested simpler methods like email or phone verification. As P5 stated, \textit{"most of the people are there for entertainment, and they just upload for fun. And at places where people usually go for fun, they don't require much information from a user. In an OTP or like email verification is kind of like enough for those platforms."}, they explained that online platforms, which do not require extensive personal information, are sufficient with simple verifications.

\section{RQ2: Design Suggestions for PHC}

\subsection{Participants' Needs for PHC Designs}
Participants expressed specific needs for PHC systems, primarily focusing on \textbf{decentralization and transparency}. P4 preferred a decentralized approach, stating, \textit{"I prefer the decentralized version just because you’re not giving all the power or like responsibility to government, although government might have all the information."} Additionally, transparency was identified as a critical requirement. P4 also noted, \textit{"I think any of this institute, if they take this responsibility, they need to be regulated about how they’re gonna handle user privacy security. They should be transparent about their process."} This emphasis on transparency and accountability highlights the need for PHC issuers to demonstrate their commitment to protecting user privacy and security as trusted issuers.

\subsection{Participants' Suggestions for PHC Designs}
Participants suggested several design improvements for PHC systems. 

\textbf{Design Theme 1: Decentralization} One suggestion focused on \textbf{decentralized data storage} to reduce the risk associated with a single point of failure Figure \ref{fig:sketch_pilot_p5}. As P5 noted, \textit{"They will be able to like the data will be stored on different platforms, and it will reduce the risk of like attack one and get all scenario." } This approach enhances PHC's security by distributing data across multiple locations. Similary, P4 drawed decentralized system, inspired by sector-based privacy policies. The participant explained that privacy policies are often structured according to specific sectors as shown in Figure \ref{fig:sketch_pilot_p4}. His idea is having a group of folks in certain entities, one of which is social media, government, and bank, instead of one institute managing or issuing the PHC. For example, PHC issuer for social media would be managed by a group of representatives from major social media companies, chosen through a democratic process.

\textbf{Design Theme 2: Surveillance} P3 proposed a combined solution involving a \textbf{third party between PHC issuer and the user} alongside \textbf{encrypted credentials} to strengthen data privacy Figure \ref{fig:sketch_pilot_p3}. They suggested introducing an intermediate to oversee verification, explaining \textit{the current system is PHC issuer directly verifying the user's information…my idea is maybe some kind of third party could be here between them." }Furthermore, P3 recommended using multi-layer encryption with multiple keys, noting \textit{”The original identification is only visible with encryption…we should have maybe two keys…so that hackers could encounter challenges the whole time to decrypt." } By involving a third party and employing advanced encryption, this suggestion aims to safeguard sensitive information while fostering trust in the PHC system. M1 also presented the government's involvement as a supervisor of PHC issuers. The participant expected the government is involved in the issuance, storage, and auditing of PHCs, helping to prevent fraud and enhance system trust as explained \textit{"The government would need to be involved in the process of PHC issuance...They do audit checks and validate the storage of data, or validate the issuance of a particular PHC."}

\textbf{Design Theme 3: Protection from Potential Attacks}
M2 showed security concern on two types of potential attacks: social attack which tricks to have users to share the credential; system attack to database. As protection to such attacks, she proposed multiple approaches can be implemented - \textit{"There are a lot of methods that's already there. So for example, protection algorithm to make the algorithm or make the system more robust. And also there's a lot of like education training things to prevent social engineering."}


\begin{figure}[!t]
 \vspace{-5pt}
	\centering
	\includegraphics[width=\linewidth]{Fig/sketch_pilot_p3.png}
 \vspace{-15pt}
	\caption{Sketch by P3: Encryption and intervention by checking organization}
\label{fig:sketch_pilot_p3}
\vspace{-15pt}
\end{figure}


\begin{figure}[!t]
 \vspace{5pt}
	\centering
	\includegraphics[width=\linewidth]{Fig/sketch_pilot_p4.png}
 \vspace{-15pt}
	\caption{Sketch by P4: Sector-based Decentralization}
\label{fig:sketch_pilot_p4}
\vspace{-15pt}
\end{figure}

\begin{figure}[!t]
 \vspace{5pt}
	\centering
	\includegraphics[width=\linewidth]{Fig/sketch_pilot_p5.png}
 \vspace{-15pt}
	\caption{Sketch by P5: Selective Access to Information}
\label{fig:sketch_pilot_p5}
\vspace{-15pt}
\end{figure}

\begin{figure}[!t]
 \vspace{5pt}
	\centering
	\includegraphics[width=\linewidth]{Fig/sketch_m1.png}
 \vspace{-15pt}
	\caption{Sketch by M1: Government involvement in PHC Issuers’ system}
\label{fig:sketch_m1}
\vspace{-15pt}
\end{figure}

\begin{figure}[!t]
 \vspace{5pt}
	\centering
	\includegraphics[width=\linewidth]{Fig/sketch_m2.png}
 \vspace{-15pt}
	\caption{Sketch by M2: Protection from potential attacks}
\label{fig:sketch_m2}
\vspace{-15pt}
\end{figure}


==> Sections/Results_RQ0.tex <==
% \section{RQ0: Current Online Identity Verification Practices}

% \textbf{Verification Across Multiple Domains} The most common online services where participants encountered identity verification processes are financial services, including online banking and investment platforms. Several participants mentioned they are required to upload government IDs (e.g., social security number, driver's license) when creating an account; as P1 said, \textit{"I use the bank I need to upload my social security number for, such as PNC Bank and Discover. I don't really remember. But I'm sure I have uploaded my social security number."} In addition to financial services, the typical applications where participants experienced verification or authentication processes include social media, government services, and healthcare platforms. 
% %This indicates that the scenarios we prepared for succeeding sessions are representative of typical user occasions. 

% \textbf{Confusion Between Verification and Authentication} Many participants did not distinguish between verification and authentication. In particular, when asked about experiences with biometric verification, they often shared daily experiences related to authentication, e.g., (P3): \textit{"It's I think most of the apps required me such fingerprints or related identification. For example, when I open my bank apps, I can just use my fingers to login to my account."} Participants indicated frequent use of fingerprints or face authentications on mobile phones. For instance, P1 mentioned stored biometric information on devices, \textit{"Because my android phone already have my fingerprint to log into my phone. And then this app just to reuse my fingerprint, which is already registered on my phone."}

% \textbf{Verification in daily life} Some of the participants shared their offline experience that required identity verification, as P1 described \textit{"So I need to check in in a hotel. I also need to show my driver's license. I don't know if that count."} 


==> old/0-Method.tex <==
 \section{Method Overview}
Building on the existing literature, it is clear that while significant progress has been made, a critical gap remains in understanding the key factors required to operationalize personhood credentials that balance privacy, security, and trustworthiness online. This challenge becomes even more pressing with the rise of increasingly advanced AI, which enables bad actors to scale their operations, exacerbating issues such as impersonation, fake identities, and non-human interactions. As outlined in Figure~\ref{fig:method}, our study comprises: (1) a competitive analysis of current verification tools and an analysis of Reddit data to identify challenges. These insights inform the design of a user study aimed at (2) investigating users’ perceptions (RQ1), identifying factors influencing their preferences for personhood credentials (RQ2), and conceptualizing a design framework (RQ3) to address these challenges.

%Please add the flow digram / RQs of different methods with a method overview. see here https://arxiv.org/pdf/2410.01817?}



\section{Formative Understanding of PHCs}

In this section, we outline our formative analysis of existing personhood verification systems, which informed the design rationale for developing our user study(Section~\ref{user-study}).

%\subsection{Competitive Analysis \& Cognitive Walkthrough}
\paragraph{Competitive Analysis.} No prior studies have explored personhood credentials systems' usability and security issues. To address this gap, we systematically consolidated metadata from both practical implementations and state-of-the-art systems, including the World app, BrightID, Proof of Humanity, Gitcoin Passport, and Federated Identities (OAuth). We chose these systems based on their popularity, diversity in platform type (centralized vs. decentralized), and relevance to the domain of digital identity\fixme{add citations of research papers from lit review}. Table~\ref{tab:identity_verification} provides an overview of different attributes of how existing systems operate and their design trade-offs. We found 15 apps categorized into six groups. Five of these were centralized, primarily government-based personhood verification systems. The data requirements for issuing credentials varied, including behavior filters, biometrics (such as face, selfie, iris, or video), social graph and vouching mechanisms, physical ID verification, and, in some cases, combinations of these methods. 

%which helps us conduct a cognitive walkthrough. 

%we analyzed 15 popular systems in terms of their features, such as issuance system (centralized vs decentralized), types of data requirements for issuing credentials, types of  service providers of those systems. 
%Our competitive analysis allowed us to explore and identify multi-criteria to assess aspects such as privacy, usability, and security

\paragraph{Cognitive Walkthough}
For the cognitive walkthrough, we focus 
%on evaluating a system's usability and privacy by simulating 
how a user would navigate and identify potential usability and security issues. Two experts (experts in UI/UX and verification systems, in our case) evaluated if users can successfully use an
application interface and complete core tasks, signing up with the application and receiving the personhood credential. While some apps are proof of concepts or can't have access, such as, Aadhar Card, Estonia's digital ID and China's social credit system, we documented the workflow based on white papers. 
%For evaluating the current verification process of some applications, we have utilized cognitive analysis of UI/UX, data requirement and privacy issue 
%We have selected some popular centralized and decentralized platforms such as World app, Bright ID, Proof of Humanity, Passport Gitcoin, Federated Identities (OAuth), Aadhar Card, Estonia's digital ID and China's social credit system . 
Working as two evaluators, we first independently generated an initial list of evaluation results of those apps while considering the following questions set.
%For cognitive analysis of UI/UX, we have considered a few questions set: 
%\tanusree{from where did we get these questions? My impression was- we are doing cognitive analysis of ui/ux and data requirement, privacy issues, questions here doesn't reflect the goal of cognitive walkthrough}
\begin{itemize}
    \item How intuitive is the registration and verification process for both new and experienced users?
    \item How effectively does the platform provide feedback during different steps of registration and verification?
    \item How do we as users felt regarding the data requirements in the verification systems?
%\end{itemize}
%The following 2 questions have been utilized for data requirement analysis
%\begin{itemize}
    \item What type of data (e.g., personal and biometric, etc) are required for issuing the credentials?
    \item In which stage, are these credentials requested from users? How we as users felt regarding the data requirements in the verification systems
%\end{itemize}
%We have also analyzed the privacy concerns using these 2 questions:
%\begin{itemize}
    \item How does the platform manage users' data to ensure users' privacy and security?
    \item What are the potential risk factors regarding users' privacy in the platform?
\end{itemize}

The competitive analysis aimed to evaluate and compare the verification processes of the \fixme{it should be a total of 15} eight selected verification systems (Table~\ref{tab:identity_verification}).
%The following predefined criteria were utilized to ensure a structured and consistent evaluation of the platforms:

% \begin{itemize}
%     \item Type of platform
%     \item Free or paid
%     \item Required data
%     \item Stage where data is required
%     \item Centralized or decentralized
%     \item Advantage
%     \item Disadvantage
%     \item UI/UX issue
%     \item Privacy related issue
% \end{itemize}
Throughout this cognitive walkthrough, (a) we conducted a qualitative assessment of the user interface and user experience, focusing on ease of use, clarity, and overall usability; (b) we created test accounts to study and asses the workflow and documented the key steps, required information and potential privacy and security issues.
% We collected data for analysis using the following approach:
% \begin{itemize}
%     \item We analyzed the user interface and the user experience qualitatively and focused on ease of use, clarity and usability.
%     \item We created test accounts to study and asses the whole account creation workflow and documented the key steps and required information.
% \end{itemize}
Finally, we structured the data according to aforementioned criteria to highlight notable differences and their implications on usability and privacy.

  %  \item We reviewed official resources such as documentation and privacy policy to evaluate privacy concerns. 

\begin{table*}[h!]
    \centering
    \begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{3cm}|l|l|}
        \hline
        \textbf{Category} & \textbf{Service Name} & \textbf{Types of insurance} & \textbf{Issuer} & \textbf{Type of Credential} & \textbf{Type of Platforms} & \textbf{Free or Paid}\\
        \hline
        \multirow{3}{*}{Behavioral filter} & CAPTCHA & Decentralized & open-source, vendor & Humanness verifier & & Free\\
        \cline{2-7}
         & reCAPTCHA & Centralized & Google & Humanness verifier & & Free\\
        \cline{2-7}
         & Idena & Decentralized & open-source & Solve flip (contextual puzzle) & & Free\\
        \hline
        \multirow{2}{*}{Biometrics} & World ID & Centralized, decentralized & World & Biometrics (iris scan) & Android, iOS & Free\\
        \cline{2-7}
        & Humanode & Decentralized & Humanode & Biometrics (face) & & Paid\\
        \hline
        Social Graph & BrightID & Decentralized & open-source & Analysis of a social graph & & Free\\
        \hline
        Social Vouching & Proof of Humanity & Decentralized & Kleros & Social vouching & & Free\\
        \hline
        \multirow{2}{*}{Decentralized Oracle} & DECO & Decentralized & Chainlink Labs & Decentralized oracle (Cryptographic proof) & & Paid\\
        \cline{2-7}
        & CANDID & Decentralized & IC3 research team & Decentralized oracle (Cryptographic proof) & & Free\\
        \hline
        \multirow{4}{*}{ID system offered by Government} & Adhar Card & Centralized & Gov & Document-based or Head Of Family-based enrollment + capture photograph of face, 10 fingerprints and 2 iris & & Free\\
        \cline{2-7}
        & Estonia e-ID & Decentralized & Gov & Passport or EU ID + digital photo of your face & & Paid\\
        \cline{2-7}
        & Chinese Credit system & Centralized & Gov & Personal credit records & & Free\\
        \cline{2-7}
        & Japan My Number Card & Centralized & Gov & Application letter from Gov + face photo or identification documents & & Free\\
        \hline
        \multirow{2}{*}{Other verification tools/products} & ID.me & Centralized & ID.me & Government-issued ID & & Free\\
        \cline{2-7}
        & Civic Pass & Decentralized & Civic & Humaness verifier, Biometric, ID & & Free\\
        \hline
        \end{tabular}
    \caption{Table of Existing Identity Verification Systems}
    
    \label{tab:identity_verification}
\end{table*}



\subsection{Results of UI/UX}
\tanusree{Silvia: why do we have only 3 apps in the analysis?Ayae created a list a long ago. please complete the analysis for all the apps from this list}  \tanusree{I am not sure why facebook is in the analysis. we talked about only including verification apps, facebook is not one of them}
\fixme{look at the Suggetsions in comment}
The eight \fixme{15 systems} systems evaluated manifest diverse approaches to user experience, emphasizing accessibility, intuitiveness, and transparency\fixme{write in active sentence or active voice, it reads like chatGPT and reviewer will think the same}. Platforms such as World App and BrightID developed on decentralized technologies, 
%though their intricate verification methods, 
including zero-knowledge proofs\fixme{add citation} and social connections \fixme{add as footnote what social connection means here and citation}, may confuse non-technical users. Proof of Humanity requires video submissions \fixme{what kind of video, is it their face? then talk about privacy, this doesn't seem to be a blockchain issue rather privacy issue}, a process potentially intimidating for individuals less familiar with blockchain platforms. 

In contrast, Federated Identities (OAuth) streamlines login processes via well-known third-party providers\fixme{who is the third-party provider for them}, ensuring ease of use for most users \fixme{is that all? }. 

Government-supported systems like Aadhaar and Estonia e-Card feature structured interfaces but come with limitations: Aadhaar’s biometric registration may challenge rural populations, while Estonia’s dependence on smart-card hardware might exclude those without the necessary devices. \fixme{add about Japan My Number Card.} 

Passport Gitcoin, focused on Web3 integration, struggles with clarity for users new to decentralized identity concepts. Finally, China’s Social Credit System delivers a seamless yet opaque experience, leaving users uncertain about the data influencing their scores.\par
Data requirements across the systems vary significantly in scope and sensitivity. Decentralized platforms like World App, BrightID, and Proof of Humanity emphasize minimal data collection but still require sensitive information, such as Ethereum addresses, social graphs, or video proofs, to ensure authenticity. Centralized systems, including Aadhaar and Estonia digital ID, require extensive personal and biometric data—fingerprints and iris scans—to ensure seamless service delivery. Passport Gitcoin, designed for Web3 wallet integration, relies on centralized storage, demanding significant user trust. Federated Identities (OAuth) achieves a balance by sharing limited data through third-party providers but this comes with the risk of overexposure. China’s Social Credit System stands out for its vast data collection, encompassing financial, social, and daily activities, raising alarm over pervasive monitoring and privacy intrusion.\par
Privacy concerns are critical across the eight systems, influenced by their data management practices. Decentralized platforms like World App and BrightID prioritize privacy, yet linking personal data to public blockchains—as seen in Proof of Humanity—poses inherent risks. Centralized systems like Aadhaar and Estonia e-Card depend on centralized databases, making them vulnerable to surveillance risks. Federated Identities (OAuth) simplifies access but could expose user data to third-party providers without explicit consent. Passport Gitcoin presents privacy challenges because users' information can be shared with third-party service providers. Meanwhile, China’s Social Credit System exemplifies extreme privacy erosion, extensively monitoring citizen behavior with minimal transparency about data use. Striking a balance between privacy and functionality remains a universal challenge for all these systems.

\fixme{citations to be added} We have evaluated 15 systems to present diverse approaches to user experience, emphasizing usability, accessibility, intuitiveness and transparency.
\fixme{citation didn't work} CAPTCHA\cite{Captcha} and reCAPTCHA\cite{reCaptcha} are 2 common human verification tools used across many websites. While CAPTCHAs add an additional step for users when they are trying to access a website, reCAPTCHAS come into play by removing any external verification. Rather, reCAPTCHAs track users' activities which has raised privacy concerns as there is lack of transparency between user and reCAPTCHA authority. Users are not sure how the tracking data will be used. Platforms such as World app\cite{WorldWhitepaper} and Bright ID\cite{BrightID} are developed on decentralized technologies which include zero-knowledge proofs but do not present a clear and concise terms and conditions and privacy policy, which may create reluctance for new users to start using them. In figure 1(a), the on-boarding screen of World App appears with a consent checkbox to obtain explicit consent from the users that they agree to the "Terms and Conditions" and acknowledge the "Privacy Notice" of World App. But the terms and conditions and privacy notice are not mentioned in the same screen, tapping on the link buttons redirects users to a different screen, thus creating an obstacle in their user journey. If the necessary terms and conditions were presented clearly and concisely on the on-boarding screen, it would have informed users about the app's policies and ensure a smoother user journey. 1(b) represents the Bright ID license agreement, but it is too long to read. Users may not have enough patience to go through the details as it is time consuming and tap the agree button to continue. But this action may create privacy risks as users don't know what type of access they are providing to the application.
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Fig/world app t&c.png}
         \caption{The terms and conditions and privacy notice are not mentioned in the World App's on-boarding screen}
         \label{fig:The terms and conditions and privacy policy are not mentioned in the World App's on-boarding screen}
     \end{subfigure}
     \hfill
     % \begin{subfigure}[b]{0.3\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{Fig/google drive.png}
     %     \caption{World App requires users to connect Google Drive for enabling backup}
     %     \label{fig:five over x}
     % \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Fig/bright id t&c.png}
         \caption{Bright ID's license agreement contains a long description which users may not want to read}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
        \caption{On-boarding screens of World App and Bright ID}
        \label{fig:three graphs}
\end{figure}
In figure 2, we can see World App requires users to connect their Google Drive to back up their world app accounts but this may lead users to providing access to their sensitive information.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{Fig/google drive.png}
    \caption{World App requires users to connect Google Drive for enabling backup}
    \label{fig:World App requires users to connect Google Drive for enabling backup}
\end{figure}
% \iffalse
% \begin{figure}
%  	\centering
%  	\includegraphics[width=0.5\linewidth]{Fig/world app t&c.png}
%  	\caption{The terms and conditions and privacy policy are not mentioned in the World App's on-boarding screen}   
%  \label{fig:The terms and conditions and privacy policy is not clearly mentioned}
%  \end{figure}
%  \begin{figure}
%  	\centering
%  	\includegraphics[width=\linewidth]{Fig/bright id t&c.png}
%  	\caption{The license agreement and privacy policy is too long to read}   
%  \label{fig:The license agreement and privacy policy is too long to read}
%  \end{figure}
% . \par
%  \begin{figure}
%  	\centering
%  	\includegraphics[width=\linewidth]{Fig/google drive.png}
%  	\caption{World App requires users to connect Google Drive for enabling backup}
    
%  \label{fig:World App asking to connect Google Drive}
%  \end{figure}


 


Proof of Humanity\cite{PoH}\cite{PoHexplainer} offers a unique approach to verification with a social identification system. But the verification process requires users to connect their cryptocurrency wallet which will be publicly linked to users' account. Thus, users' wallet holdings and transaction history will be linked to users' identity which users may not prefer. In contrast, Federated Identities OAuth\cite{OAuth} provides streamlined login process via well known third-party service provides, also known as identity providers such as Google, Facebook etc. It ensures ease of use as users need to specify the identity provider during the login or authentication process and grant access to their specific data. But, data is shared across multiple platform which may raise privacy concerns among users. DECO\cite{zhang2020deco} and CanDID\cite{maram2021candid} are decentralized and privacy preserving oracle protocols where DECO allows users to prove the authenticity of website data obtained over TLS (Transport Layer Security) without revealing sensitive information. But Oracle has access to users' data which pose as a privacy risk. CanDID provides users with control of their own credentials but privacy depends on the honesty and integrity of verifiers and decentralized identity validators. Idena\cite{idenaWhitepaper}, Humanode\cite{Humanode} and Civic Pass\cite{CivicPass} - all are blockchain based person identification system where Idena performs validation by conducting flip tests and Humanode and Civic Pass are developed on crypto-biometric network. Though Idena does not collect any personally identifiable information, the behavioral data collected can be used in future for pattern analysis. Humanode and Civic pass both require biometric verification (face scan) which can create concerns among users about how their sensitive credential (face) will be managed by the systems. It is noteworthy that, most of the platforms are decentralized (World App, Bright ID, Proof of Humanity, Idena, Humanode, Civic), some requiring cryptocurrency wallet (Proof of Humanity, Civic Pass) and some requiring biometric verification (Proof of Humanity, Humanode, Civic Pass).    %citations to be added
\par
Government issued identity documents such as Aadhaar Card, Estonia's e-ID, China's social credit system and Japan's My Number Card are controlled and managed by central government. Citizens' sensitive credential can be at high risk if the government's security system is not robust enough to prevent any kind of hacking or data breaching. China's social credit system monitors citizen data extensively without maintaining complete transparency about data use and management. ID.me is another online identity network that enables individuals to verify their legal identity digitally. But privacy concerns arises as a single company holds a large amount of personal data and users have limited control over their data. %citations to be added
\par
Usability across these different platforms are critical. CAPTCHAs have become increasingly difficult to solve, often leading users to leave the website or platform without completing their user journey. Accessibility remains another issue as visually impaired users are unable to solve any CAPTCHA that is text or image based. reCAPTCHA comes with the solution of these problems but trading of users' privacy as users' data is being tracked down by the authority. From Figure 3 and 4, it is apparent that World app and Bright ID provide a simple and intuitive account creation form but an introductory video or step by step guide would be more helpful to guide users to navigate throughout the applications and perform necessary actions.
 \begin{figure}
 	\centering
 	\includegraphics[width=\linewidth]{Fig/world app account creation.png}
 	\caption{World App's account creation process is simple but doesn't inform users about how they should navigate or use the app \fixme{silvia, is there a reason you added all these UIs? why all of the uis are randomly placed, I shared examples so many times, i am not seeing anything I gave instruction.}}
 \label{fig:World App's on-boarding process}
 \end{figure}
 
 \begin{figure}
 	\centering
 	\includegraphics[width=\linewidth]{Fig/bright id account creation.png}
 	\caption{The "Create my BrightID" process in the Bright ID app is straightforward but lacks guidance on how users should navigate or utilize the app effectively. \fixme{explain why these screenshots are important to add from cognitive walkthrough. caption itself should be self explanatory with text explaining in the main body}}
    
 \label{fig:Bright ID's on-boarding process}
 \end{figure}
The principle of error prevention could make the user journey of registration in Proof of Humanity more user-friendly. As there is no option to correct or update any mistake, it may increase user frustration. Idena's validation test (flip test) (Figure 4) can be inconvenient for new users as they may struggle to find the meaningful story in the provided time and collect points to validate them.
 \begin{figure}
 	\centering
 	\includegraphics[width=\linewidth]{Fig/idena.png}
 	\caption{Idena validation test interface requiring users to select meaningful stories within a time limit which can be challenging for new users \fixme{anyone reading this caption would not understand anything}}
    
 \label{fig:Selecting meaningful story for validation process on Idena}
 \end{figure}
The platforms requiring video selfie or face scan (Proof of Humanity, Humanode, Civic Pass) may create another challenging situation for users as proper lighting and optimal devices are necessary for taking the appropriate photo or video for biometric verification. Aadhaar card\cite{Aadhaar}\cite{AadhaarEnrollment}, Estonia's e-ID and Japan's My Number Card are all government based credentials but completing all the formalities and getting the card takes a long time, sometimes creating user frustration. The existing systems and platforms that we have evaluated can hardly strike a balance between privacy, functionality and usability.   %citations to be added


% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=\linewidth]{Fig/world app.png}
% 	\caption{New account creation process in  World App}
    
% \label{fig:New account creation process in  World App}
% \end{figure}
% \begin{figure}[!t]
% 	\centering
% 	\includegraphics[width=\linewidth]{Fig/bright id.png}
% 	\caption{New account creation process in  Bright ID}
    
% \label{fig:New account creation process in  Bright ID}
% \end{figure}

\subsection{Reddit Analysis}
%\tanusree{ishan to add}
We first collected \fixme{X} posts and  \fixme{X} comments on December 24th, 2024, using the Python Reddit API Wrapper (PRAW)~\footnote{https://praw.readthedocs.io/en/stable/}. We gathered the data from various relevant subreddits, ensuring a broad and comprehensive understanding of what users discuss on identify verification or personhood verification. Through qualitative analysis of this Reddit data, we were able to uncover detailed insights into the rich and prevalent usage of verification systems. This analysis highlighted users' current usage, potential challenges and risks they encounter. These findings provide a solid foundation to explore these themes further in subsequent in-depth interviews.

\paragraph{Data Collection}
 To comprehensively cover content related to our research questions on personhood verification, we first created a list of search keywords by identifying close terminologies related to \textit{``personhood verification''} (general keywords) and \textit{``bot check''} (technology-focused keywords), etc. We utilized a combination of general and technology-focused keywords in our search. We employed general terms such as Personhood Verification, Identity Proof, Human Check and Bot Check. These keywords were designed to capture posts authored by or discussing personhood verification. For the technology focus, we used terms such as \fixme{add}. These keywords targeted discussions specifically about the use of popular tools and platforms. We conducted open searches combining these keywords across Reddit to gather data from various subreddits.
 Other than open searches, we also applied specific criteria to select subreddits, ensuring comprehensive coverage of relevant discussions: these subreddits should focus either on the personhood verification community or technology. We chose subreddits with the most active users online during our browsing sessions. The full list of subreddits and search keywords used is detailed in Table\fixme{need to find out the subreddit most prevalent discussing these topic}. 

\paragraph{Analysis}
Two researchers reviewed each post and categorized related posts or comments into five overarching high-level themes: \fixme{need to add after data analysis}. Within these categories, 53 level-2 themes were identified, such as \fixme{need to add after data analysis}. During the analysis process, researchers regularly convene to discuss discrepancies and emerging themes in the codebook, aiming to reach a consensus. These categories allowed us to investigate RQ2 and partially address RQ1. 

\subsection{Results}
% \tanusree{ishan to add}

\section{ User Study Method}
\label{user-study}
This section outlines the method for exploring users' perceptions and preferences of personhood credentials. We conducted semi-structured interviews with \fixme{21} participants from the US, the EU/UK in October 2024.
%We started with a round of pilot studies (n=5) to validate the interview protocol. Based on the findings of pilot studies, we revised the interview protocol and conducted the final round of interviews (n=17). 
The study was approved by the Institutional Review Board (IRB).

\subsection{Participant Recruitment}
We recruited participants through (1) social media posts, (2) online crowdsourcing platforms, including CloudResearch and Prolific. Respondents were invited to our study if they met the selection criteria: a) 18 years or older and b) living in the US or the EU/UK. Participation was voluntary, and participants were allowed to quit anytime. Each participant received a \$20 Amazon e-gift card upon completing an hour-and-a-half interview.

\subsection{Participants}
We interviewed \fixme{21} participants, 9 from the US and 12 from the EU/UK. The majority of the participants (70\%) were in the age range of 25-34, followed by 17\% were 35-44 years old. The participants were from the United States and various countries, namely Spain, Sweden, Germany, New Zealand, and the United Kingdom. Participants had different backgrounds of education levels, with 82\% of participants holding a Bachelor’s degree and 64\% holding a graduate degree. 64\% of participants had CS background, while 52\% of them had a technology background. All participants reported using online services that required them to verify their identity. Table~\ref{table:demographics} presents the demographics of our participants. We refer to participants as P1,. . . ,21.



\subsection{Semi-Structured Interview Procedure} \label{sec:study_protocol}
%\fixme{explain in details why the study designed in a certain way. please read papers to learn more. data minimization and advertisement paper. The method section is too bland. We have a wonderful study design. Scenario-specific study design, describe scenarios and why chose this scenario. Mainly method should include all design rationale, and example questions when necessary to clarify your rational}

We started with a round of pilot (Appendix~\ref{pilot}) studies (n=5) to validate the interview protocol. Based on the findings of pilot studies, we revised the interview protocol

\textbf{Open Ended Discussion.} We designed the interview script based on our research questions outlined in the introduction section~\ref{sec:introduction}. We added the interview script to the supplementary materials. At the beginning of the study, we received the participants’ consent to conduct the study. Once they agreed, we proceeded with a semi-structured interview. The study protocol was structured according to the following sections: (1) Current practices regarding digital identity verification; (2) Prior understanding of PHC; (3) Watching an educational video on PHC and post understanding of PHC (4) Scenario-based session to investigate users' perceptions of PHC; (5) Design session to explore users' preferences and design implications; (6) Post-survey.

In the first section, We first asked a set of questions to understand participants' current practices of online platforms they often use and the types of identity verification methods they had experience with. This is to understand their familiarity with different types of verification, such as biometrics, physical IDs, etc, and methods that might have worked well based on their prior experience.
%of online identity verification. When participants mentioned certain types of online services that required identity verification, we inquired about their experience with verification method. Was it easy to use, or did you run into any issues?"} We further inquired about any challenges participants faced with identity verification - \textit{"Did you encounter any challenges when using this method?"} 
%If biometrics didn’t naturally come up in prior discussions, we prompted to consider them- \textit{"Have you ever used services where you had to verify yourself through face, fingerprints, or iris scans, or other biometrics?"} If they mentioned any experience with biometric verification, we followed up with questions like- \textit{"What worked well? Were there any concerns you had?"}
We then asked about participants' current understanding of personhood credentials either from prior knowledge or from intuition by just hearing the word, for instance, we asked-\textit{``Do you know the term 'Personhood Credentials'?  Can you explain what it means by just hearing the term?''} We also asked if they knew how personhood credentials work, particularly how it has been handled by the different services they use. In the pilot interviews, The majority of the participants could not provide substantial responses on their understanding 
of how personhood credentials work, before starting the second part of the interview, we showed them an informational video on personhood credentials.
%Most of the participants were unfamiliar with this term, so we then asked \textit{ Can you explain what you think it means by just hearing the term?"} 
%Before proceeding with the third section of the interview, we assessed participants' understanding of PHC with knowledge questions.
We showed them an introduction video on PHC. The video provides an overview of PHCs, covering their definition, the steps involved in issuing and using them, and implications of it online services. Based on the discussion of former literature\cite{adler2024personhood}, we designed the video with clear, easy-to-understand visuals and audio to make the concepts accessible to users. We created a survey to assess participants' understanding of PHC before and after showing the video, including, the same knowledge questions. We also asked some open-ended questions to evaluate whether our introduction video helped participants better understand PHC \textit{''How would you explain your understanding of personhood credentials?''} 
%We further asked what benefits and concerns came to mind for them.

In the second section, we focused on scenario-based discussions, exploring specific applications of PHC to understand participants' perceptions and identify ways to improve PHC design for various services. We examined the following six scenarios: (1) Financial service, (2) Healthcare service, (3) Social Media, (4) LLM applications, (5) Government Portal, and (6) Employment Background Check.
We covered a wide range of use cases of online identity verification via these six scenarios since they encompass diverse user needs, security levels, and privacy requirements. \fixme{please see the comment with iffalse tag and make it concise, we talked about it before}
\iffalse
Firstly, financial system is a critical scenario for identity verification where high level of security protections are expected as exemplified by KYC. Thus, such services continue to develop transformative digital identity verification to ensure the security and integrity of financial transactions\cite{parate2023digital}. The second scenario is healthcare systems, which also have high privacy requirements due to the confidentiality of medical data. The pandemic has accelerated the adoption of online healthcare services and in response to this digital transformation, the recent study has proposed blockchain-based decentralized identity management systems \cite{javed2021health}. Thirdly, we consider the scenario of social media, which faces the critical challenges of online identity as shown in spreading misinformation and harmful content from fake or anonymous accounts \cite{ceylan2023sharing}. The fourth scenario is designed with a specific context of interacting with Large language models (LLMs). The former study discussed vulnerability in dialog-based systems where adversaries can exploit the training process to introduce toxicity into responses \cite{weeks2023first}. Thus, such vulnerabilities indicate identity verification may also be important for LLM applications. Fifth, government services are familiar situations that require people to verify their identity. Various countries have developed their own electronic ID schemes \cite{stalla2018gdpr}. Lastly, we also cover the scenario of employment background checks needing precise identity verification to ensure the reliability of applicants. The current background check system involves vulnerable processes that increase the risk of identity theft and unauthorized data access.\cite{blowers2013national}. Such challenges underline the relevance of PHCs, which can mitigate risks by providing a secure framework for verification.
%\ayae{included citation}
\fi
We have also incorporated various types of credentials for each scenario to maintain diversity in our discussion with participants as shown in \ref{table:scenario}. For instance,
%we  We have multiple existing verification methods, including 
humanness verification (e.g., selfie, video call), document-based verification (e.g., government-issued ID), and biometrics information. We selected types of credentials for each scenario based on former literature and existing PHC as explained in the section \ref{subsec:verification_practice}. %\fixme{cite worldcoin, and other app and literature}. \fixme{from here to end of this paragraph ---These needs to go to the literature review section on the current usecase of PHC. And only 2 line summarizing why you chose the diverse type of credential data and refer to the literature section}


%% Let me find the former literature to explain why we select these credentials
For each of the six scenarios, we explored participants' perceptions of using PHC in hypothetical situations that align with the research focus as well as to help participants can relate PHC concepts to real-world applications. This is particularly useful for this study where where user perceptions and expectation under specific conditions are crucial to devising solutions \cite{carroll2003making}.
%\fixme{cite scenario method paper from jack caroll}.\ayae{reflected}
We asked about their feelings, perceived benefit and risks. We also nudge them to think about any privacy and security perception around using PHC and types of data (e.g., iris, face, government id, etc )involved in issuing PHC. 
%began by asking \textit{"How did you feel about using PHC to verify your identity when opening your bank account?"} To dive deeper, we also asked about potential benefits:\textit{"What potential benefits do you see in using PHC in this online banking context?"}. We also inquired about these aspects- \textit{"Do you think using PHC improves the security of your bank account? Why?", "Did this method of identity verification make you feel more confident about your privacy? why?"} Additionally, we discussed their comfort levels for providing credentials (e.g., Government-issued ID, biometric information) and asked about any concerns about data collection-\textit{"Were you comfortable providing your government-issued ID and using facial recognition? Why?"}

%%% column: scenario, credential, service providers.
\begin{table*}[h!]
\centering
\caption{Overview of PHC Application Scenarios}
\label{table:scenario}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\textbf{Scenario} & \textbf{Service Provider} & \textbf{Types of Credential} \\
\hline
Financial Service & Bank & Passport or Driver’s license, Face scan \cite{yousefi2024digital}\\
% \hline
Healthcare Service & Hospital & Health insurance card,  Fingerprint \cite{chen2012non,fatima2019biometric,jahan2017robust}\\
% \hline
Social Media & Companies & National identity card, Video selfie \cite{instagramWaysVerify, metaTypesID,instagramTypesID} \\
% \hline
LLM Application & Companies & Iris scan \cite{WorldWhitepaper, worldHumanness}\\
% \hline
Government Service & Government & Driver’s license or National identity card \cite{LogingovVerify}\\
% \hline
Employment Background Check & Third-party companies & Tax identification card, Fingerprint\cite{cole2009suspect}\\
\hline
\end{tabular}%
%}
% \vspace{0.5em}
\label{tab:scenarios}
\end{table*}



%\textbf{Design Session.}
%\fixme{need to explain how and why you design the design session, where you designed, how participants were unstructured and so on.} \ayae{reflected in the following paragraph}

In third section, we investigated participants' preferences for PHC in context of who issue PHC, and what types of data are needed to issue PHC to address RQ2. First. we asked about the preferred types of credentials and the preferred stakeholders to issue and manage their PHC- \textit{``What types of credential would you prefer to use as personhood verification? ; Which organizations or stakeholders would you prefer to issue and manage your PHC?''} However, these questions alone can only find optimal ways within the scope of currently existing options and cannot generate new design implications. Therefore, we instructed participants to brainstorm solutions by sketching their ideas on Zoom whiteboard or pen and paper, using a think-aloud protocol. Nevertheless, it is difficult to develop new ideas from scratch, so we shared sketch notes to kick off the sketch session when necessary, as shown in \ref{fig:sketchnote}. By arranging the components that constitute the architecture of PHCs on the left side, we lowered the barrier to sketching. Additionally, we described the main issues or concerns that the participants identified during the interview at the top of the sketch notes. Participants can develop their ideas at the center of the whiteboard by locating the above components or creating new shapes, lines, or text boxes for their sketches. 

Lastly, we introduced the decentralized PHC system architecture with another instructional video. The rationale for why we introduced it after the sketch session is that participants may organically come up with the idea of decentralized systems on their own, and we intended to avoid priming them. Then, we asked them to explain their understanding of the decentralized PHC and preferred issuance system (centralized or decentralized)- \textit{"Would you prefer to get multiple PHCs from different issuers depending on the situation or application you're using, or would you rather have a single PHC from one issuer?"}

\textbf{Post-Survey.}
%%\fixme{need to explain how and why you design the design session, where you designed, how participants were unstructured and so on.}
For the closing of our interviews, we conducted a post-survey to understand their PHC preference quantitatively. It included questions about credential preference, issuer preference, and issuance system preference for the same scenarios (e.g., financial, medical, etc) we considered in section 2 in our interview. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{Fig/zoom_whiteboard.png}
	\caption{Zoom Whiteboard: Pre-arranged components like the PHC issuer and database are placed on the left of the whiteboard, while potential concerns or risks suggested by participants during interviews are noted as topics in the top right. %\fixme{figure caption needs to be self explanatory by itself}
    }
\label{fig:sketchnote}
\end{figure}

\subsection{Data Analysis}
Once we got permission from the participants, we obtained interview data through the audio recording and transcription on Zoom. We analyzed these transcribed scripts through thematic analysis \cite{Braun2012-sz, Fereday2006-yv}. Firstly, all of the pilot interview data was coded by two researchers independently. Then, we compared and developed new codes until we got a consistent codebook. Following this, both coders coded 20\% of the interview data of the main study. We finalized the codebook by discussing the coding to reach agreements. Lastly, we divided the remaining data and coded them. After both researchers completed coding for all interviews, they cross-checked each other’s coded transcripts and found no inconsistencies. Lower-level codes were then grouped into sub-themes, from which main themes were identified. Lastly, these codes were organized into broader categories. Our inter-coder reliability (0.90) indicated a reasonable agreement between the researchers.


\begin{table*}[h]
\centering
\caption{Participant demographics and background.}
%\fixme{add the participants you completed so far}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l l l l l l l}
\hline
\textit{Participant ID} & \textit{Gender} & \textit{Age} & \textit{Country of residence} & \textit{Education} & \textit{CS background}  & \textit{Technology background} &\textit{Residency duration} \\
\hline
P1 & Male & 25-34 & the US & Master's degree & Yes & Yes &3-5 years\\
P2 & Female & 25-34 & the US & Master's degree & Yes & Yes & 1-3 years\\
P3 & Female & 25-34 & the UK & Master's degree & Yes & No & 1-3 years\\
P4 & Female & 35-44 & the UK & Some college, but no degree & Yes & Yes & Over 10 years \\
P5 & Male & 25-34 & the US & Doctoral degree & Yes & Yes & 5-10 years \\
P6 & Male & 35-44 & the US & Less than a high school diploma & No & No & Over 10 years \\
P7 & Male & 25-34 & the US & Doctoral degree & Yes & Yes & 3-5 years\\
P8 & Male & 45-54 & the US & Bachelor's degree & Yes & Yes & Over 10 years \\
P9 & Female & 25-34 & New Zealand & Master's degree & No  &  No &  Over 10 years\\
P10 & Male & 25-34 & the US & Master's degree & No & No & Over 10 years\\
P11 & Female & 25-34 & the UK & Bachelor's degree & No & No & Over 10 years\\
P12 & Male & 18-24 & the UK & Master's degree & Yes & Yes & 1-3 years\\
P13 & Male & 35-44 & the UK & Bachelor's degree & Yes & No & Over 10 years\\
P14 & Male & 25-34 & Sweden & High school graduate & No & No & Over 10 years \\
P15 & Female & 25-34 & Spain & Master's degree & Yes & Yes & Over 10 years \\
P16 & Female & 25-34 & Germany & Master's degree & Yes & Yes & Over 10 years \\
P17 & Female & 25-34 & Spain & Doctoral degree & No & No & Over 10 years \\
P18 & Female & 35-44 & USA & Bachelor's degree & No & Yes & Over 10 years \\
P19 & Female & 25-34 & Germany & Master's degree & Yes & Yes & 3-5 years \\
P20 & Male & 25-34 & Hungary & Master's degree & Yes & No & 3-5 years \\
P21 & Male & 35-44 & USA & Bachelor's degree & Yes & No & 5-10 years \\
P22 & Female & 18-24 & France & Master's degree & Yes & Yes & Less than 1 year\\
\hline
\end{tabular}%
}
\label{table:demographics}
\end{table*}


==> old/Result-old.tex <==


\section{RQ1: Users’ Current Impression of PHC}

%\subsection{Current Online Identity Verification Practices}

\textbf{Current Verification Practices: Multi Data and Context Verification.} 
When discussing services that required identity verification, participants most commonly mentioned financial services, including online banking and investment platforms, as well as health services, government-related processes, cross-border regional verifications, and two-factor authentication (2FA) used by various institutions. The discussion highlighted both digital and physical forms of verification. Several participants mentioned they are required to upload government IDs (e.g., social security number, driver's license) when creating an account- as P7 said--\textit{``For Robinhood, it asked for uploading my government issued IDs like driver's license and passport.''} 
%In addition to financial services, the applications where participants experienced verification processes include a wide range of applications. 
Similarly, P2 explained their verification experience in the government services requiring multiple information \textit{``I remember, if you go use like government related service, filing the text files, they would require you to verify your identity through your face.''} Beyond financial and government services, identity verification has also become essential in marketplace apps,
%that rely on trust to facilitate peer-to-peer transactions. 
P1 illustrated this trend with Airbnb, explaining  \textit{``If you do book an Airbnb, at least as a renter, you would need to verify your government id before being eligible to book your first stay.''} 
%This indicates that the scenarios we prepared for succeeding sessions are representative of typical user occasions. 

%\textbf{Confusion Between Verification and Authentication} Many participants did not distinguish between verification and authentication. In particular, when asked about experiences with biometric verification, they often shared daily experiences related to authentication, e.g., (P3): \textit{"It's I think most of the apps required me such fingerprints or related identification. For example, when I open my bank apps, I can just use my fingers to login to my account."} Participants indicated frequent use of fingerprints or face authentications on mobile phones. For instance, P1 mentioned stored biometric information on devices, \textit{"Because my android phone already have my fingerprint to log into my phone. And then this app just to reuse my fingerprint, which is already registered on my phone."}

\textbf{How Users Evaluate the Trustworthiness of Stakeholders} When discussing the current verification process, participants often indicated that there are organizations they can trust and others they cannot. Thus, we asked how or why they have trust with specific stakeholders. P5 explained his trust in banks comes from regulatory aspects: \textit{"They are being monitored by federal agencies. Their activities are monitored. They are under a lot of regulations. So there is a monitoring system that is tracking banks, at least Major Banks or Banks that I know of and other financial services they are under a lot of regulations."} P4 highlighted another aspect resulting in their trust in banks,  which is that the accessible customer support, stating \textit{"You know what sort of steps have taken so you could probably have a read of that, and any concerns that you might have. So you probably always have the opportunity that you could always speak to them first, because obviously they probably have agents available that you could speak to about any concerns. "} On the other hand, we observed that many participants expressed distrust towards social media platforms. P3 shared a formative experience of her social media account almost being hacked, noting \textit{"I've had people experience...Who then tried to get like hack into my account. So the one hacker would hack one person's account, and because, obviously, in your social media, you have access to other people's accounts as well, like I've had people send me really dodgy links, which I knew like instantly, that if I clicked on that link, it would mean that my account would get hacked as well."} Some participants elaborated on how they evaluate the trustworthiness of companies or stakeholders when they share their sensitive information in general. P6 reflected \textit{"I guess if the company was suggested to me, or I was referred to the company through the services of like Capital One or a big company that's been around forever. That would give more validity to me."} P7 provided insight from his own experience with a suspicious verification process, saying \textit{"I do a lot of research… What I did was I went and searched on the Internet. So I went on Reddit, and I looked for different keywords, and my conclusion was that it's a very standard process. It's not like the dealership wants to collect the social security for themselves. They wanted to do the background check, and they wanted to see if the information that they provided was matching with my information from the US. "}

%\textbf{Offline Verification in Daily Life} Some of the participants shared their offline experience that required identity verification, especially in the context of international travel and immigration procedures,  as P3 described \textit{"So in the past I've had to use my fingerprints, for example, when I came to the UK. When I had to renew my passport in the embassy of my country, they would take my fingerprint there. So they would take a photo of my current passport, and then they would take a photo of myself, but then they would also require me to give my fingerprints as well."}  


\subsection{Perceived Benefits of Personhood Credentials}
%\fixme{there needs to be titles of sub-themes under this benefit, it's hard to read. Sub-themes could be -- convenience of not carrying physical id, etc -- whatever unique /interesting subthemes came up in the interview}
\textbf{Verify Uniqueness with Reduced Exposure of Personal Information} Participants identified a range of benefits, the most frequently mentioned being the reduction of personal information exposure. P4 expressed \textit{"I think the what I glean from it was there was to provide without giving away too much personal information, but it can still sort of verify your uniqueness."} In addition to this, several participants highlighted the benefits related to online identity crisis with AI. P11 summarized the benefits of PHC, \textit{"Personhood credentials is a way in which a person can confirm that they are not a bot or an AI, and that they're a real person without giving away their personally identifiable information."} P11 also extended the discussion on this point to online malicious attacks, \textit{"I think that it will tackle like fake accounts, multiple accounts and bots massively. And I can see it being used like, really broadly, because you're not giving away any really important information... And having to get this identification through, like your government, or something works really well, because you don't mind giving them the information. And then, the kind of redacted information that you give to social media sites, increases safety and stuff, but doesn't put your data at risk."} P1 explained increased confidence in privacy through PHCs for unfamiliar entities \textit{"All of that information doesn't need to be filled in each time, you fill a form for submission and the potential conference that if I am signing up for an account with a 3rd party, which I have not heard before. I'm not comfortable with even in the case of a breach. They would not have access to my personal information, but just rather the identifier id. So that would be something I'd be comfortable with. "}

\textbf{Efficiency of Verification Process} Another key benefit highlighted by participants was the efficiency of verification process. P3 emphasized the convenience of less repeated verification, stating, \textit{"Having an easier login from a trusted source. So it's ease of access for the user." }


\subsection{Perceived Concerns of Personhood Credentials}
%\fixme{there needs to be titles of sub themes under this benefit, it's hard to read }
Participants expressed various concerns, primarily revolving around data security and trustworthiness of PHC issuers. 

\textbf{PHC Issuer Being Hacked or Leaked} One of the most frequently mentioned concerns was the potential risk of PHC issuers being hacked or experiencing data leaks. As P8 explained, \textit{"However, the problem with having one identity or one credential for everything is, if that credential is stolen, all of your accounts are at risk, and that is where I don't like the idea of one verification credentials. So if I use one verification for my bank and email and Facebook and Facebook gets hacked and they steal that credential and well, now, my bank and email accounts are also at risk."} It highlights participants' fears that the concentration of sensitive data with PHC issuers could have severe consequences for malicious attacks.

%\textbf{Data Handling by PHC Issuers} Another significant concern was how PHC issuers manage and handle the credential data they collected. Participants showed uncertainties regarding what happens to their personal information after verification and whether it is securely stored or potentially mishandled. For example, P4 shared that \textit{"I'm not sure if they tell us explicitly how they're gonna use, do they going to share our information with 3rd party or with government. If they ask for it, I'm not sure about that. These are my concerns."}

%\textbf{Centralized PHC} Several participants expressed concerns over the centralized power held by PHC issuers, which they feared could lead to misuse or overextension of control. P4 commented \textit{"But I think there's a concern on the other side that they're gonna be one kind of you're gonna give all your information to a small group or an institution. So they have the power that can be abused later."} illustrating the apprehension about the concentration of power in the hands of a single entity as a PHC issuer.

\textbf{Trustworthiness of PHC Issuer} The issue of trustworthiness in PHC issuers was also discussed, with participants expressing doubts about the reliability of the entities managing their data. Some worried whether these issuers could be trusted to protect their personal information and maintain their privacy. P7 described \textit{"My only concern is, how do we trust the Phc Am I using it? Yeah, because if if they are the one entity who handles all these kind of information, and if they are collecting everything about us from the government. And whether this entity is considered like a NGO, or that's a governmental body, or that if that's a private sector, so these are like some nuances about how to define or how to build this kind of issuer, because we have these giant issuers like Equifax or like these giant companies who are handling credits or those kind of financial aspect of the US structure. And they're like giants. They have these kind of monopoly over how they handle things. Is it going to be something similar? If so, how people can trust them? I don't want to share my personal information anymore, with like some random website...But how the way that the issuer can be understood? I think that would be the decision factor for users to start engaging with the system."}

\subsection{Motivational Experiences for Using PHC}
When discussing the benefits of PHCs, participants shared their experiences with deceptive online activities stemming from digital identity crises ranging from bots to scams. P10 explained the issue of bot accounts on social media, noting \textit{"I get random bots following me on my twitter a lot which I'm assuming. If they had this PHC Implemented, we would probably see a reduction in those types of bots...I'm assuming there's bots on Instagram as well, and I'm sure most social media accounts is probably bots."} P11 also reflected on fake news spread by bots, \textit{"I know that bots and AI and stuff are utilized quite a lot on social media sites, and to spread like fake news, and to support certain people's agendas and the kind of a tool that that are used in order to."} Accordingly, identity verification is recognized as a key area of concern in the context of social media platforms for end-users due to the proliferation of bot accounts and the dissemination of fake news. 

In addition, some participants emphasized the significance of identity verification in relation to cryptocurrency. P13 stated scams in cryptocurrency, \textit{"I think with cryptocurrency, everyone's scamming everyone all the time...And the companies who do the id verification basically decided it might be legally difficult. So they just stop. So that's probably the main problem I've had."} P12 indicated trade-off between privacy and traceability in crypto wallets, \textit{"I don't really like identity you put in your facial verification, or your Id or your driver's license on trust. But for Binance, Bybit and KuCoin, they actually request that because it's actually a big company or anything. But I'll see it's just a very diverse app that you can do a lot of things on. It needs the privacy of other people. It needs the privacy of other people and yours to cooperate because of scams and fraud."}

\subsection{Context Matters for Users' Preference}
As outlined in the method section \ref{sec:study_protocol}, we explored participants’ perceptions and preferences regarding PHC across five distinct scenarios. Participants’ responses indicated the necessity of verification methods depending on the specific scenario. In some contexts, they considered PHC unnecessary and suggested simpler methods like email or phone verification. As P5 stated, \textit{"I love to talk, to, chatgpt, and bard about weird stuff, and I think a lot of people like to talk to them about weird stuff. And so I would like the option to not log in via biometrics, and have a lesser experience and not have my identity tied to it. So I personally, I would not like to have my identity tied to my chat Gpt, or my bard, or Gemini."}, they explained that online platforms, which do not require extensive personal information, are sufficient with simple verifications.

\subsection{Perception Before \& After Educational Video}
As discussed in the method section \ref{sec:study_protocol}, we revisited questions about participants' understanding of PHC to compare their responses before and after watching the educational video to assess whether the video impacted their original knowledge of PHC. 

\textbf{Pre-understanding: Guessed it as one of the verification methods} As all participants have never heard of PHC, we prompted them to interpret the term based solely on its wording. Most of them inferred that it referred to another type of person identification. For example, P3 commented \textit{" It can be anything that would point to one single individual that would differentiate that individual from others."} When participants expressed how PHC identify person's uniqueness, their thoughts has a variety, ranging from basic information such as address or age to more advanced approaches like Multi-factor authentication or knowledge-based questions.

\textbf{Post-understanding: Involvement of trusted entity} When asked to explain their understanding of PHC, P13 noted, \textit{"So it sounds like, basically, you it's similar to how you verify things before. Like you use a biometrics and your government Id. But then you get a personal key. You do it with like a trusted organization rather than each individual. And then you can use that key for all the different services you use."} P1 elaborated PHC process as a shift of the verification entity, \textit{" I'd say we are sort of moving the verification burden from the user side to a service provider side where they have access to our data, and they have access to the token that's assigned to each person that's unique. And that's easily like traceable across online platforms. and this token is used for verification with 3rd parties, where they don't get access to your personal data, but they only use this service provider to give them the authenticity that you are a real user."} These suggest that the role of the PHC issuer is recognized as a crucial component of PHC.

\textbf{Where Misunderstandings Can Arise in PHC}
We observed that users sometimes misunderstood PHCs. These misconceptions represent critical points that should be carefully addressed in communication when aiming for the widespread adoption of PHC in the future. P10 explained the benefit of PHC, stating \textit{"I am thinking that imagine you are a criminal or an online criminal. For example, with some records that you are not allowed to use some services online. For federal government, they need to verify your credentials to be able to track you or just not allow you to do activities."} This comment was interpreted as PHC enhancing traceability to assist in criminal investigations. Such potential traceability was also mentioned in the context of tech companies tracking data, saying \textit{"But what is more of a concern for me is that some of these big tech companies like Google, like Facebook, like even Apple, Amazon. They use that information to track my searches and activities."} However, PHCs are fundamentally intended to serve as a means of anonymously verifying users' personhood without compromising their privacy. 


%\textbf{Post-understanding: Found similarities with other technologies} P5 interpreted the term as a verification method based on personal characteristics, which differ from person to person, such as behavioral patterns, commenting \textit{"It's like, personality based or like activities humans particularly perform. It sounds similar to the pattern of people walking. Those are also things people use for verification."} After watching the video, he updated his perception of PHC \textit{"I thought it was similar to SSL technology. Like in SSL, they will give the certificate to 3rd party who encrypts and has those certificates. To maintain their integrity, they will pass on the kind of certificate to web browsers. So when a user goes through a particular website, they will be able to cross-verify using the public keys available."}, linking it to technologies such as SSL, which uses encryption and hashing for certificates.

